Maximum Entropy Differential Dynamic Programming

In this paper, we present a novel maximum entropy formulation of the Differential Dynamic Programming algorithm and derive two variants using unimodal and multimodal value functions parameterizations. By combining the maximum entropy Bellman equations with a particular approximation of the cost function, we are able to obtain a new formulation of Differential Dynamic Programming which is able to escape from local minima via exploration with a multimodal policy. To demonstrate the efficacy of the proposed algorithm, we provide experimental results using four systems on tasks that are represented by cost functions with multiple local minima and compare them against vanilla Differential Dynamic Programming. Furthermore, we discuss connections with previous work on the linearly solvable stochastic control framework and its extensions in relation to compositionality.

==> plots/quad/old_plots/grid_plot.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/MER_00_.pdf}
    \end{subfigure}%
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/MER_02_.pdf}
    \end{subfigure}%
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/MER_04_.pdf}
    \end{subfigure}
    \ac{MME-DDP}
    \par\vspace{1em} % Vertical spacing between the rows.
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/ER_00_.pdf}
    \end{subfigure}%
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/ER_02_.pdf}
    \end{subfigure}%
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/ER_04_.pdf}
    \end{subfigure}
    \ac{ME-DDP}
    \par\vspace{1em} % Vertical spacing between the rows.
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/Vanilla_00_.pdf}
    \end{subfigure}%
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/Vanilla_02_.pdf}
    \end{subfigure}%
    \begin{subfigure}[c]{0.33\columnwidth}
         \centering
         \includegraphics[width=0.99\textwidth]{plots/quad/Vanilla_04_.pdf}
    \end{subfigure}
    Vanilla-DDP
    \caption{
    Position trajectories for the quadcopter problem from 16 different seeds.
    Only \ac{MME-DDP} is able to avoid the local minima in
    the center which intersects all four of the obstacles in all $16$ seeds.
    }
    \label{fig:sims:quad_states}
\end{figure}


==> scratch.tex <==

\begin{equation} \label{eq:er_ddp:optimal_policy}
    \pi^*(\delta u | \delta x) \propto
    \exp \left( -\frac{1}{\alpha} \Big[
        \frac{1}{2} (\delta u - \delta u^*)\T Q_{uu} (\delta u - \delta u^*) \Big]
        \right),
\end{equation}
where the optimal deviation from the nominal controls

As we will see later,
the above equation becomes easier to work with when considering the 
exponential transformation of the original cost and value functions.
For notational simplicity, define $\expalph$ to be the following function:
\begin{equation}
    \expalph(y) \coloneqq \exp \Big(-\frac{1}{\alpha} y \Big).
\end{equation}
% Then, we define the exponential transformations of the cost and value functions to be
We now define the following terms





plugging the above into the form of the optimal policy \eqref{eq:er_hjb:optimal_policy},
we obtain the optimal policy
We see that the optimal policy \eqref{eq:er_ddp:optimal_policy} is a multivariate Gaussian distribution with mean $\bar{x} + \delta u^*$ and
covariance $\alpha Q_{uu}^{-1}$.
Plugging this into the Taylor expansion of the
Bellman equation \eqref{eq:er_hjb:raw_bellman}, we see that
where the terms $\bar{V}$, $V_{H}$, $V_x$ and $V_{xx}$ have the form
Note that the update rules for , which results from the Shannon entropy of a Gaussian distribution and
approaches $0$ as $\alpha \to 0$.

Performing a Taylor expansion of $Q \coloneqq V'(f(x,u)) + l(x,u)$ in the Bellman equation \eqref{eq:er_hjb:raw_bellman} with respect to $x$ and $u$, we obtain the following
\begin{gather}
    V'(f(x,u)) + l(x,u) \approx V'(f(\bar{x},\bar{u})) + l(\bar{x}, \bar{u}) + \delta Q, \\
    %%%%%%%%%%%%%%%%%5
    \delta Q \coloneqq
    \begin{bmatrix}Q_x \\ Q_u\end{bmatrix}\T \begin{bmatrix}\delta x \\ \delta u\end{bmatrix}
    + \frac{1}{2}
      \begin{bmatrix}\delta x \\ \delta u\end{bmatrix}\T
      \begin{bmatrix}Q_{xx} & Q_{xu} \\ Q_{ux} & Q_{uu} \end{bmatrix}
      \begin{bmatrix}\delta x \\ \delta u\end{bmatrix}. \label{eq:me_ddp:delta_Q}
\end{gather}
By completing the square and using \eqref{eq:er_hjb:optimal_policy}
